SurgeoNet: Realtime 3D Pose Estimation of Articulated Surgical Instruments from Stereo Images using a Synthetically-trained Network

Surgery monitoring in Mixed Reality (MR) environments has recently received substantial focus due to its importance in image-based decisions, skill assessment, and robot-assisted surgery. Tracking hands and articulated surgical instruments is crucial for the success of these applications. Due to the lack of annotated datasets and the complexity of the task, only a few works have addressed this problem. In this work, we present SurgeoNet, a real-time neural network pipeline to accurately detect and track surgical instruments from a stereo VR view. Our multi-stage approach is inspired by state-of-the-art neural-network architectural design, like YOLO and Transformers. We demonstrate the generalization capabilities of SurgeoNet in challenging real-world scenarios, achieved solely through training on synthetic data. The approach can be easily extended to any new set of articulated surgical instruments. SurgeoNet's code and data are publicly available.

==> rebuttal.tex <==
% The rebuttal should in total be 4000 characters -including spaces and new lines- starting after this comment. the current draft is >4000 chars


First, we would like to thank all the reviewers for taking the time to provide invaluable feedback on our work. We also thank them for acknowledging the problem's novelty, the effectiveness and efficiency of our method, and the paper's comprehensiveness and clarity.

% (R1) Reproducibility:  

% We plan to release the training and testing code publicly which will provide all details about the implementation. 

(R1): MR devices have depth sensors 

We relaxed the assumption of having a depth channel available as this would add a constraint on the applicability of our method to general stereo-RGB views. 

(R1, R6): Robustness to hand occlusions 

To improve robustness to hand occlusion, we use temporal smoothing and tracking which stabilize the output from the network. This helps mitigate the wrong results given by the YOLO network when the object is temporally occluded by the hand. However, we observed that under severe, prolonged occlusions, the model failed to locate the instruments as the task became more challenging, even for the human eye to classify and determine their keypoints. 

% (R6): Comparison to related works

% We think of our work as an initial experiment (step forward) towards tracking articulated surgical instruments which will open the door for future researchers to study the problem. We are aware of some methods that track surgical instruments like Hein et. al. (2021) which we mention in our introduction. 
% The lack of a benchmark dataset for surgical instruments makes direct comparison to other methods difficult. Furthermore, those methods mainly focus on a tiny set of completely rigid instruments e.g. scalpel or drill, with no mention of articulated instruments. Therefore, testing their methods would require a cumbersome amount of changes to their input and output modalities and retraining steps. The same goes for the other 6 DoF pose estimation methods. The other suggested papers to compare with, like Gsaxner et. al. (2019) and von Atzigen et. al. (2022), cover different surgery monitoring problems.

% (R6): Details on YOLOv8 and ByteTrack

% We provide in the following the requested details, although they are not part of our contributions. More extensive detail can be found in the paper's citations.
% YOLOv8 is a convolutional network that builds upon earlier versions of YOLO (Redmon et. al. 2018) with advanced backbone and nick architectures for improved feature extraction. ByteTrack (Zhang et. al. 2022) is a MOT algorithm that improves over previous MOT algorithms by associating almost all detections instead of only the high-scoring ones which improved the tracking in case of occlusions. ByteTrack predicts the new location of tracks from previous frames using Kalman Fitlers. It then uses similarity metrics like IoU and Re-ID to associate new bounding boxes to the tracks. This way it can keep unique IDs for the tracks.

(R6): Runtime evaluation and GPU inference

Figure 4a shows that we can achieve more speed when reducing the model size or image resolution while losing accuracy. The user can choose between accuracy or speed when running the demo. At the moment, we are working with a PCVR headset which means it should be connected to a PC and hence can use its GPU power to run the demo. 

(R6): Performance with blood and smoke

We thank the reviewer for their suggestion as we could simulate smoke and blood as texture in the synthetic data and finetune the network to handle those cases. The current purpose of our project is to provide an educational demo for medical students that assists them in learning to deal with surgical instruments.

(R6): Evaluation on real images

In future work, we plan to publish a new dataset of real frames with annotations and it can serve for training and evaluation of surgical instrument tracking. At the moment, we provide confusion matrix evaluation on real images along with qualitative results.



% (ADD ABOUT TEMPORAL)
% As part of our experiments, we rendered the shape of a hand with different textures around the rendered instruments to encourage YOLO to find the instruments under occlusions. This experiment improved YOLO's performance slightly in partial occlusions. 
% Some extra sentences that can be used 

% Moreover, most XR headsets and medical setups in operation rooms share the same limitation of ourheadset.
% We will mention the HMD-Pose method in the camera-ready version. 

% (R3): the variety of objects and recognizing the fine differences   

% Our synthetic dataset can be easily extended to new instruments by rendering frames using instrument meshes. The confusion matrix on real frames in Figure 5 shows the ability of the network in distinguishing between similar scissor-like instruments most of the time.
